Decouple knowledge from parameters for plug-and-play language modeling

Pre-trained language models(PLM) have made impressive results in various NLP tasks. It has been revealed that one of the key factors to their success is the parameters of these models implicitly learn all kinds of knowledge during pre-training. However, encoding knowledge implicitly in the model parameters has two fundamental drawbacks. First, the knowledge is neither editable nor scalable once the model is trained, which is especially problematic in that knowledge is consistently evolving. Second, it lacks interpretability and prevents humans from understanding which knowledge PLM requires for a certain problem. In this paper, we introduce PlugLM, a pre-training model with differentiable plug-in memory(DPM). The key intuition is to decouple the knowledge storage from model parameters with an editable and scalable key-value memory and leverage knowledge in an explainable manner by knowledge retrieval in the DPM. To justify this design choice, we conduct evaluations in three settings including: (1) domain adaptation. PlugLM obtains 3.95 F1 improvements across four domains on average without any in-domain pre-training. (2) knowledge update. PlugLM could absorb new knowledge in a training-free way after pre-training is done. (3) in-task knowledge learning. PlugLM could be further improved by incorporating training samples into DPM with knowledge prompting.

==> content/0-abstract.tex <==
Large-scale pre-trained language models~(PLM) have made impressive results in a wide range of NLP tasks and it has been revealed that one of the key factors to their success is the parameters of these models implicitly learn various types of knowledge in the pre-training corpus.
However, encoding knowledge implicitly in the model parameters has two fundamental drawbacks. First, the knowledge is neither editable nor scalable once the model is trained, which is especially problematic in that knowledge is consistently evolving. Second, it lacks interpretability and prevents us from understanding what kind of knowledge PLM needs to solve a certain task. In this paper, we introduce \model, a pre-training model with differentiable plug-in memory~(DPM). The key intuition behind is to decouple the knowledge storage from model parameters with an editable and scalable key-value memory and leverage knowledge in an explainable manner by knowledge retrieval in the \memory. 
We conduct extensive experiments under various settings to justify this design choice. In domain adaptation setting, \model could be easily adapted to different domains with pluggable in-domain memory---obtaining 3.95 F1 improvements across four domains, without any in-domain training. \model could also keep absorbing new knowledge after pre-training is done by knowledge updating operation in the \memory without re-training. Finally, we show that by incorporating training samples into \memory with knowledge prompting, \model could further be improved by the instruction of in-task knowledge.

==> content/1-introduction.tex <==
Large-scale pre-trained language models~(PLM)~\citep{peters-etal-2018-deep,devlin-etal-2019-bert,radford2018improving} have become a revolutionary breakthrough in NLP area. Optimized by carefully designed self-supervised objectives on unlabeled corpus and fine-tuned on downstream tasks, PLMs perform remarkably well in a wide range of NLP benchmarks. Recent studies~\citep{warstadt2019investigating,petroni2019language} have revealed that one of the key factors to the success of PLMs is that the parameters of these models implicitly learn various types of knowledge in the pre-training corpus. Owing to these learned syntactic, semantic, factual and commonsense knowledge, PLMs show great understanding, generalization and reasoning abilities in multiple downstream tasks~\citep{rogers2020primer,izacard2022few}. As \citet{geva2021transformer} pointed out, the feed-forward layers~(FFN), constituting two-thirds of a transformer model's parameters, are essentially key-value memories and store all kinds of knowledge of PLM. The first linear layer of FFN acts like a set of sparsely activated keys detecting input patterns while the second is the corresponding value. To aggressively capture more knowledge, larger PLMs are continuously proposed, from 110M BERT~\citep{devlin-etal-2019-bert} to 530B MT-NLG~\citep{smith2022using}, yet PLM has not reached upper bound~\citep{ouyang2022training}. 

However, a fundamental question still remains: \textbf{For PLM, is it the optimal way to implicitly encode knowledge in its parameters? } We argue that the implicit knowledge encoding approach has two fundamental drawbacks. 
First, the learned knowledge is neither editable nor scalable once the model is trained. Nevertheless, world knowledge is actually infinite and evolving. We thus would never expect an ever-large model to capture all the knowledge in its parameters and to be continuously re-trained for the newly coming one. 
Second, the current PLMs lack interpretability at the knowledge level. Implicit knowledge encoding fails to provide provenance for model’s prediction and makes PLM a black box preventing us from understanding which knowledge does PLMs require for a certain task. 

In this work, we propose a novel architecture of PLM, \model, which decouples the knowledge storage from model parameters and explicitly leverages the knowledge in an explainable manner. As shown in Figure~\ref{fig:model}, we balance the functionality of FFN layer with a differentiable plug-in key-value memory~(\memory), which is highly scalable as well as editable. Each slot of \memory encodes the knowledge to a pair of key and value, and thus we can explicitly retrieve the required knowledge from \memory rather than unnamed vectors in FFN.


To justify the design choice of decoupling the knowledge from parameters, we conduct extensive evaluations under different settings. 
In the domain adaptation setting, \model could be easily adapted to different domains with pluggable in-domain memory---obtaining 3.95 F1 improvements across four domains on average and up to 11.55 F1 improvement on \arccite citation intent classification dataset, without any in-domain pre-training. 
In the knowledge update setting, \model could absorb new knowledge after pre-training is done in a training-free way by knowledge updating operation in the \memory, with an improvement up to 4 F1 scores in \texttt{LINNAEUS} NER dataset. 
\model could further be improved by incorporating training samples into \memory with knowledge prompting as a kind of in-task knowledge.


\begin{figure*}[t]
		\centering
		\begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/model.pdf}
        \end{subfigure}%
		\caption{Overview of our \model. We replace FFN in PLM with a Differentiable Plug-in key-value Memory~(DPM) by which PLM could store and leverage knowledge in an explainable manner.}
		\label{fig:model}
\end{figure*}

==> content/2-related_work.tex <==
\paragraph{Investigating FFN} 
Feed-forward layers constitute two-thirds of a transformer model's parameters and are essential to unveil modern PLMs~\citep{geva2021transformer,geva2022transformer}. A surge of works have investigated the knowledge captured by FFN~\citep{dai2022knowledge,meng2022locating,geva2021transformer,geva2022transformer,jiang2020can,yao2022kformer,wallat2020bertnesia}. Based on the view that FFN is essentially an unnormalized key-value memory network, \citet{dai2022knowledge} detects knowledge neurons in FFN and edit specific factual knowledge without fine-tuning. \citet{meng2022locating} modifies FFN weights to update specific factual associations using Rank-One Model Editing. \citet{yao2022kformer} injects knowledge into the FFN via BM25. \citet{dai2022neural} and \citet{lample2019large} enhance the model by expanding the size of FFN with extra trainable keys and values. 
%One main difference of our model is that the \memory is grounded: each key-value pair is associated with one concrete knowledge rather than unnamed vectors.

\paragraph{Knowledge-Augmented Language Model} There are two lines of works to equip PLM with knowledge. 
The first is introduce additional Knowledge Graph~(KG) and knowledge-based training signal~(e.g., entity linking) into the language model pre-training, like ERNIE~\citep{zhang2019ernie,sun2019ernie}, KnowBERT~\citep{peters2019knowledge} and KEPLER~\citep{wang2021kepler}. Another line of works adopt retrieval mechanism to incorporate knowledge, either symbolic~\citep{verga2021adaptable,agarwal2021knowledge,fevry2020entities} or texual~\citep{guu2020retrieval,lewis2020retrieval,borgeaud2022improving,lewis2020pre,verga2021adaptable,de2021mention}. They formulate the task as retrieve then predict process by using extra neural dense retriever~(BERT) or sparse retriever~(BM25) to find most relevant supporting knowledge and combine it with input using either concatenation~\citep{guu2020retrieval} or attention methods~\citep{de2021mention,wu2021memorizing,fevry2020entities,chen2022augmenting}. 

\model differs from previous works in that we do not try to equip the model with additional knowledge to perform knowledge-intensive tasks. The key insight is to transform FFN architecture into deep retrieval in the interest of decoupling the knowledge, which would otherwise be stored in the parameters, with an editable and scalable \memory and leverage knowledge in an explainable manner.

==> content/3-method.tex <==
\subsection{Preliminary}
\paragraph{Feed-forward Layers} Transformer~\citep{vaswani2017attention}, the backbone for all PLMs, is made of stacked self-attention~(Self-Attn) and feed-forward~(FFN) layers. The former captures the contextual interaction among inputs and the latter process each input independently.  Let $x \in \mathbb{R}^{d_{1}}$ be a vector as input, the FFN could be formulated as:
\begin{equation}
\label{equation:ffn}
	\text{FFN}(x) = f(x\cdot W_{1}^\top)\cdot W_{2}
\end{equation}
where $W_{1},W_{2}\in \mathbb{R}^{d_2\times d_1}$ and $f$ is the activation function.

\paragraph{Key-Value Memory Network}
The Key-Value Memory Network~\citep{weston2014memory,sukhbaatar2015end} corresponds to $d_2$ key-value pairs and each key/value is a vector in $\mathbb{R}^{d_1}$. They are the generalization of the way knowledge is stored~(e.g., context in Dialogue~\citep{eric2017key} and documents in QA~\citep{miller2016key}). For an input $x \in \mathbb{R}^{d_{1}}$, there are two stages for a key-value memory network. First, the lookup~(addressing) stage would compute the matching degree between $x$ and each key. In the second stage, $x$ would be transformed by the weighted sum of values according to the distribution of the matching degree in the first stage. We can formally define it as:
\begin{equation}
\label{memorynetwork}
	\text{MemoryNetwork}(x) = \text{softmax}(x\cdot K^\top)\cdot V
\end{equation}
where $K,V\in \mathbb{R}^{d_2\times d_1}$. Comparing equation (\ref{equation:ffn}) and (\ref{memorynetwork}), we could find that the FFN is an unnormalized version of MemoryNetwork. The keys in FFN are pattern detectors and would be activated only when certain patterns occur in the input. This explains how FFN stores knowledge in a key-value manner~\citep{geva2021transformer,sukhbaatar2019augmenting}. 

\subsection{Overall Architecture}
The overall architecture of \model is illustrated in Figure~\ref{fig:model}. Because FFN is essentially a key-value memory network~\citep{geva2021transformer,dai2022knowledge,meng2022locating}, \model creatively decouples the knowledge storage from model parameters by replacing\footnote{Because different layers in transformer capture different knowledge, the lower layer for shallow patterns while the upper layers for more semantic ones~\citep{geva2021transformer,jawahar-etal-2019-bert}, we only consider replacing FFN in Top-L layers with \memory while keeping FFN in the lower layers untouched to encode the intrinsic language understanding knowledge as detailed in \S\ref{sec:tuning_model}.} FFN with a Differential Plug-in key-value Memory, DPM~(\S\ref{section:dpm_construction}) and conducting knowledge retrieval in DPM with knowledge attention~(\S\ref{section:memory_fusion}) for explicit knowledge usage instead of storing all knowledge implicitly in the model parameters. In \S\ref{section:training}, we detailedly explain how \model is trained in both pre-training and fine-tuning stages. 

\subsubsection{Differential Plug-in Memory}  
\label{section:dpm_construction}
In this paper, we view each knowledge $d_{n} = \{t^1_{n},t^2_{n},...,t^{|d_{n}|}_{n}\}$ as consecutive tokens from unlabeled corpora as in \citet{guu2020retrieval}. For each $d_n$, we get its dense representation $h_n$ from a knowledge encoder $\text{KnowEncoder}(\cdot)$:
 \begin{equation}
	h_n = \text{AttnPooling}(\text{E}_{\text{Token}}(d_n)+\text{E}_{\text{Pos}}(d_n))
\end{equation}
where AttentivePooling function~\citep{xu2021fusing,Humeau2020Poly-encoders:} corresponds to a trainable pattern detector aggregating information from a sequence of input. And $\text{E}_{\text{Token}}$ and $\text{E}_{\text{Pos}}$ denote token embedding and positional embedding. Then we use two independent mapping functions to project $h_n$ to the key space and value space:
\begin{align}
	\quad K_n = W_k \cdot h_n \quad\quad	V_n = W_v \cdot h_n
\end{align}
where $W_k$ and $W_v$ are trainable parameters. And DPM is a triplet of $\langle \mathbb{D},\mathbb{K},\mathbb{V} \rangle$:
\begin{align}
	\mathbb{D} &= \{d_1,d_2,...,d_{|\mathbb{D}|}\} \\
	\mathbb{K} &= \{K_1,K_2,...,K_{|\mathbb{D}|}\}\\
	\mathbb{V} &= \{V_1,V_2,...,V_{|\mathbb{D}|}\}	
\end{align}

%\subsubsection{Knowledge Encoder} 
%\label{section:knowledge_encoder}
%$\text{KnowEnc}_{\theta}(\cdot)$, parameterized by $\theta$, would convert a sequence of tokens into dense representation which is supposed to have the properties of alignment and uniformity~\citep{wang2020understanding}. 
%In this paper, we choose the following function. For a given knowledge $d_n$:
%\begin{equation}
%	h_n = \text{AttnPooling}(\text{E}_{\text{Token}}(d_n)+\text{E}_{\text{Pos}}(d_n))
%\end{equation}


\subsubsection{Memory Fusion} 
\label{section:memory_fusion}
For hidden states $h\in {\mathbb{R}^{l\times d}}$ from Self-Attn, FFN would transform $h$ with unnormalized key-value memory as in Equation~(\ref{equation:ffn}). Our key insight is that instead of interacting with unnamed vectors in FFN, we conduct Maximum Inner Product Search~(MIPS) to retrieve named knowledge from $\langle \mathbb{D},\mathbb{K},\mathbb{V} \rangle$ where each triplet corresponds to one knowledge along with its key and value representation. For $h$, we first get its sentence-level representation $z$ by an attentive pooling function $z=\text{AttentivePooling}(h)$, then we use $z$ as the query vector to $\langle \mathbb{D},\mathbb{K},\mathbb{V} \rangle$ and get Top-N knowledge $\mathbb{D}_{z}$ along with corresponding values $\mathbb{V}_{z}$:
\begin{align}
	\mathbb{K}_{z} &= \text{Top-N}(\text{MIPS}(z,\mathbb{K})) \\
	\mathbb{V}_{z} &= \{V_{i}\ \text{if}\ K_{i}\ \text{in}\ \mathbb{K}_{z}\} \\
	\mathbb{D}_{z}&= \{D_{i}\ \text{if}\ K_{i}\ \text{in}\ \mathbb{K}_{z}\}
\end{align}
where Top-N also corresponds to the indexing operation. With $\mathbb{K}_{z}$ and $\mathbb{V}_{z}$, following~\citet{vaswani2017attention}, we use knowledge attention to fuse retrieved knowledge into our model:
\begin{align}
 	\text{Attention}(h,\!\mathbb{K}_{z},\!\mathbb{V}_{z}\!)\!=\!\text{softmax}(\!\frac{h\mathbb{K}_{z}^\top}{\sqrt{d}}\!)\mathbb{V}_{z}
\end{align}
where $d$ is the head dimension.
By knowledge retrieval and fusion, we explore an interpretable way to incorporate knowledge into the model where $\mathbb{D}_{z}$ is the actual knowledge that PLM would leverage. And direct modification on $\mathbb{D}$ without changing model parameters empowers \model with much flexibility and scalability in domain adaptation~(\S\ref{sec:domain_adaptation}) and knowledge update  ~(\S\ref{sec:knowledge_update}) scenarios. 



\subsubsection{Training}
\label{section:training}
The backbone of our model is a multi-layer bidirectional transformer encoder~\citep{devlin-etal-2019-bert}. There are two phases in our framework: pre-training and fine-tuning. In the pre-training phase, to make the whole training process end-to-end trainable, we use asynchronous index refreshing to optimize our model as done in \citet{guu2020retrieval} and \citet{cai2021neural}. Concretely, we update the indices of DPM every T steps. The MIPS results are based on the stale index while the scores of selected Top-N results are recomputed using $\text{KnowEncoder}(\cdot)$ which facilitates the gradient flow back to memory. The training objective is Masked Language Modeling~\citep{devlin-etal-2019-bert} where we randomly mask tokens in a sentence and ask our model to predict it. In the pre-training phase, Wikipedia is chosen as the source of knowledge and in the domain adaptation fine-tuning stage, corpora from other domains are treated as knowledge sources detailed in $\S$\ref{sec:domain_adaptation}.  More details about model architecture and pre-training are shown in Appendix~\ref{appendix:pretraining_details}. In the fine-tuning phase, the $\mathbb{K}$ and $\mathbb{V}$ of DPM are fixed, and we view it as an editable and scalable knowledge lookup table.












==> content/4-experiment.tex <==
\model mainly tries to decouple the knowledge storage from parameters and leverage knowledge in an explainable way. We conduct comprehensive experiments to show the superiority of this novel architecture: we could easily adapt the model to different domains without in-domain pre-training by switching DPM~(\S\ref{section:domain_adaptive_post_training} and \S\ref{section:in_domain_pre_training}), alleviate catastrophic forgetting by storing DPM~(\S\ref{section:domain_adaptive_post_training}), inject new knowledge into the model by enlarging DPM~(\S\ref{sec:knowledge_update}), further enhance the model by injecting in-task knowledge into DPM~(\S\ref{sec:example_base_learning}) and unveil the black-box PLM with direct access to the knowledge retrieved from DPM~(Appendix~\ref{appendix:case_study}). We also carefully examine each key design in \model and point the direction for future work in \S\ref{sec:tuning_model}.

%First, in \S\ref{sec:domain_adaptation} we demonstrate the advantage of \model in domain adaptation setting by flexibly switching domain-specific \memory without changing model parameters. 
%Second, in \S\ref{sec:knowledge_update} we show \model can adjust to evolving knowledge with knowledge updating operation on $\langle \mathbb{D},\mathbb{K},\mathbb{V} \rangle$. 
%In \S\ref{sec:example_base_learning}, we show that with carefully designed knowledge prompting, \model could further improve its performance by enlarging the scope of knowledge to include training samples as in-task knowledge. 
%
\subsection{\model for Domain Adaptation}
\label{sec:domain_adaptation}
Learning robust and transferable representation has been the core of language model pre-training~\citep{peters2019knowledge}. For the general-purposed PLM to generalize well on domain-specific tasks, endowing the model with domain knowledge via in-domain training remains the go-to approach~\citep{gururangan2020don,whang2020effective,zhang-etal-2020-multi-stage}.
In this section, we show that without any in-domain pre-training, \model could flexibly adapt to multiple domains with domain-specific \memory. For the existing PLM encoding knowledge in parameters, this is a challenging task in that it can not guarantee the generalization across multiple domains due to catastrophic forgetting~\citep{kirkpatrick2017overcoming} and sometimes it is even computationally unaffordable to keep training the super large models~\citep{smith2022using,brown2020language}. 

We consider two adaptation scenarios: domain adaptive post-training and in-domain pre-training. The former is conducted after PLM was trained on the general domain and the latter trains a domain-specific PLM from scratch.

\input{content/tables/dapt_result}
\subsubsection{Domain Adaptive Post-Training}
\label{section:domain_adaptive_post_training}


\paragraph{Experimental Setting} Following \citet{gururangan2020don}, we conduct experiments on four domains: \med, \cs, \news and \reviews across eight domain-specific downstream tasks, in both low and high resource settings. More details can be found in Appendix~\ref{appendix:dapt_data}. When fine-tuning, we pass the final [CLS] representation to a task-specific head as in \citet{devlin-etal-2019-bert}.

We have the following baselines:~\textbf{WikiBERT} uses the architecture of $\text{BERT}_{base}$~\citep{devlin-etal-2019-bert} and is pre-trained on Wikipedia. To adapt WikiBERT to other domains, we use DAPT following the training setting in \citet{gururangan2019variational}. \textbf{REALM}~\citep{guu2020retrieval} and ~\textbf{\model} are models that have an external knowledge base and can be simply adapted to other domains with a different base. We have two adaptation strategies: \underline{DAA}, short for Domain Adaptive Addition, appends domain knowledge to the knowledge base, and \underline{DAR}, Domain Adaptive Replacement, replaces general knowledge with domain-specific knowledge in the knowledge base.

We also include the results of \underline{$\lnot$DAPT}, \underline{$\lnot$DAA} and \underline{DACT}. The former two use irrelevant domain corpora for post-training and knowledge base construction, which are used to test the robustness of the adaptation method and rule out the factor that improvements might be attributed simply to exposure to more data\footnote{Following \citet{gururangan2020don}, we use the following irrelevant domain mapping: for \news, we use a \cs LM; for \reviews, a \med LM; for \cs, a  \news LM; for \med, a \reviews LM.}. 
For DACT, Domain Adaptive Continual Training, we sequentially use DAPT for WikiBERT in multiple domains in the hope that it can capture and store knowledge from various domains in a lifelong learning way~\citep{rostami2021lifelong}.

\paragraph{Experimental Results} The results are shown in Table~\ref{tab:dapt_result}. The Avg.Cost is the cost for adaptation measured by hour. For WikiBERT, it's the time to post-train  model in domain-specific corpus. For REALM and \model, it is the time to encode domain knowledge into the knowledge base. We can observe: (1)~In-domain training helps model better generalize to tasks requiring domain knowledge while irrelevant knowledge misleads the model and causes performance degradation. And by comparing $\lnot$DAPT and $\lnot$DAA, it shows that models with external knowledge base~(\model and REALM) are more robust when faced with noisy out-of-domain knowledge. (2)~For the model that implicitly encodes knowledge in the parameters, it fails to generalize across domains as the result of DACT indicates. For example, we keep training WikiBERT in \news domain after DAPT in \cs domain and fine-tune it on the \cs downstream tasks. It performs on par with model that is never exposed to \cs domain~($\lnot$DAPT). \model could alleviate this catastrophic forgetting problem by storing all kinds of knowledge in \memory and using it in a plug-and-play manner. (3)~Direct modification on external memory helps \model efficiently and effectively adapt to different domains without in-domain training. In 254$\times$ less time compared with DAPT and in 40$\times$ less time compared with REALM, \model significantly outperforms DAPT and REALM-based methods.

To further understand \model, in Figure~\ref{fig:knowledge_distribution}, we present a visualization for the distribution of actual retrieved knowledge for DAA, DAR and original \model. A clear pattern here is that with more domain knowledge involved, the model performs better~(63.77, 72.51 and 75.32) and remarkably, although pre-trained on the general domain, the \model has managed to learn what to retrieve when there are both general knowledge and domain-specific knowledge in \memory shown in DAA visualization.

\begin{figure*}[t]
		\centering
		\begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=0.9\linewidth,height=0.28\linewidth]{figs/vis.pdf}
        \end{subfigure}%
		\caption{Knowledge retrieval visualization. We randomly sample 50 samples from \arccite test set and check what kind of knowledge does \model use to solve CS-specific tasks. Each column is one sample and the row is the index of retrieved knowledge in \memory. Their corresponding F1 scores are 63.77, 72.51 and 75.32.}
		\label{fig:knowledge_distribution}
\end{figure*}
\input{content/tables/squad_result}
\subsubsection{In-domain Pre-training}
\label{section:in_domain_pre_training}

In-domain pre-training is another line of work for domain-specific PLM training from scratch like BioBERT~\citep{Lee2019BioBERTAP}, SciBERT~\citep{beltagy2019scibert} and FinBERT~\citep{araci2019finbert}. 
\paragraph{Experimental Setting} In this section, we choose the biomedical domain and compare \model with model in the architecture of $\text{BERT}_{base}$, pre-trained on the general domain, Wikipedia~(i.e. WikiBERT) and pre-trained on the biomedical domain, Pubmed~(i.e. PubmedBERT). The statistics of datasets and pre-training details are listed in Appendix~\ref{appendix:pretraining_data}.
We test two kinds of abilities of these PLMs. First, we test how they perform in biomed-relevant downstream tasks. Specifically, we conduct experiments on eight representative biomedical NER datasets which aim at recognizing domain-specific proper nouns in the biomedical corpus. Then we test their general language understanding ability in \texttt{GLUE}~\citep{wang2018glue} and \texttt{SQUAD}~\citep{rajpurkar2016squad,rajpurkar2018know}. For \texttt{SQUAD} and \texttt{GLUE}, the \memory is constructed from Wikipedia, and for biomedical NER, \memory is from PubMed~\citep{canese2013pubmed}.
\paragraph{Experimental Results} The results are shown in Table~\ref{tab:ner_result}.  Both pre-trained on the Wikipedia, \model outperforms WikiBERT in 8/8 NER tasks with average 1.75 F1 scores by simply switching the knowledge domain of \memory. \model also gives comparable results with PubmedBERT in \texttt{BC4CHEMD}, \texttt{JNLPBA} and \texttt{LINNAEUS} datasets. Although PubmedBERT works well for biomedical tasks, it shows less general language understanding ability and underperforms WikiBERT and \model in \texttt{GLUE}~(Table~\ref{tab:glue_result}) and \texttt{SQUAD}~(Table~\ref{tab:squad_result}), especially in low resource scenario~(i.e., \texttt{RTE}, \texttt{COLA} and \texttt{MRPC} datasets). With \memory, \model shows great flexibility and performs well in both general domain and biomedical domain. In Appendix~\ref{appendix:case_study}, we give concrete cases of \model with respect to the retrieved knowledge.


\input{content/tables/ner_result}

\input{content/tables/glue_result}



\subsection{Knowledge Update} 
\label{sec:knowledge_update}
Since the world is not fixed as a snapshot once the pre-training corpus is collected, the current PLM, no matter how large it is, fails to adapt to this changing world. For colossal PLMs like GPT-3~\citep{brown2020language} and MT-NLG~\citep{smith2022using}, efficiently fine-tuning for downstream tasks remains an open challenge, let alone re-training it on the newly coming knowledge.

\paragraph{Experimental Setting} In this section, we show that \model can efficiently absorb new knowledge by updating the $\langle \mathbb{D},\mathbb{K},\mathbb{V} \rangle$ without re-training. We consider the following two settings. (1) We only pre-train \model with limited data and gradually enlarge the \memory with unseen knowledge when fine-tuning. (2) We pre-train \model with full general-domain data and ask the model to perform domain adaptation in DAR manner by gradually increasing domain knowledge in $\langle \mathbb{D},\mathbb{K},\mathbb{V} \rangle$.

\paragraph{Experimental Results} The results are shown in Figure~\ref{fig:knowledge_upadte_qa},\ref{fig:knowledge_upadte_cls}. For the first setting, we test on QA~(\texttt{SQUAD}) and Sentiment Classification tasks~(\texttt{SST-2}). Both WikiBERT and \model are pre-trained with only 1/4 Wikipedia corpus. We have the following observations: 
(1)~\model trained with limited data already outperforms WikiBERT in both tasks~(0.39 EM in QA and 0.59 Accuracy in classification) which verifies the effectiveness of \model in low-resource setting; 
(2) A consistent pattern across two tasks verifies \model could absorb new knowledge simply by adding more slots in  $\langle \mathbb{D},\mathbb{K},\mathbb{V} \rangle$ without heavy re-training.

For the second setting, Figure~\ref{fig:knowledge_upadte_ner} also shows our model can absorb new cross-domain knowledge under adaptation setting. It achieves a higher F1 score on the \texttt{LINNAEUS} NER dataset with increasingly more biomed-specific knowledge injected.



\begin{figure*}[t]
		\centering
		\begin{subfigure}{0.3\textwidth}
            \centering
            \includegraphics[width=0.9\linewidth,height=0.9\linewidth]{figs/squad.pdf}
            \caption{QA results.}
            \label{fig:knowledge_upadte_qa}
        \end{subfigure}%
		\begin{subfigure}{0.3\textwidth}
            \centering
            \includegraphics[width=0.9\linewidth,height=0.9\linewidth]{figs/sst2.pdf}
            \caption{Classification results.}
            \label{fig:knowledge_upadte_cls}
        \end{subfigure}%
		\begin{subfigure}{0.3\textwidth}
            \centering
            \includegraphics[width=0.9\linewidth,height=0.9\linewidth]{figs/ner.pdf}
            \caption{NER in adaptation setting.}
            \label{fig:knowledge_upadte_ner}
        \end{subfigure}%
		\caption{Knowledge update results in QA, Sentiment Classification and NER. 
        }
		\label{fig:knowledge_update}
\end{figure*}





\subsection{In-task Knowledge}
\label{sec:example_base_learning}
Inspired by \citet{brown2020language,khandelwal2019generalization} and \citet{cheng2022neural}, the training samples can also be viewed as a kind of in-task knowledge. In this section, we broaden the scope of \memory knowledge by including the training samples. 

\paragraph{Experimental Setting} Since the knowledge from Wikipedia is a textual description from domain experts~(e.g., \textit{``Machine learning (ML) is a field of, ..."}) while the training sample from a Question-answering NLI dataset is in the form of [Q, A, Label], this surface form distribution shift may affect the knowledge retrieval, we consider the following injection methods. (1)~Concate. We directly concatenate each training sample as a long string in the form of ``Q [SEP] A [SEP] Label" and append this to \memory. (2)~Tagged. To build the connection between model inputs and \memory, we tag each training sample by prepending a special token~([Tagged]), and use these tagged samples in both \memory and as model input. 
(3)~Knowledge Prompting. Inspired by prompting method~\citep{liu2021pre,schick2021exploiting}, we transfer in-task knowledge to knowledge in the form of Wikipedia by a natural language prompting. For example, in \texttt{QNLI} dataset, we transform [Q, A, Label] with the following prompting: ``The first sentence (doesn't) entail(s) with the second. The first sentence is [Q] and the second is [A]". We choose moderate-sized \texttt{QNLI} and \texttt{QQP} tasks because in-task knowledge injection doesn't apply to low-resource setting in our preliminary experiments. 
\paragraph{Experimental Results} The result is shown in Table~\ref{tab:in-task_knowledge}.  We can observe that \model has managed to learn from in-task knowledge and the surface-form of knowledge actually impact the model performance. Concatenation of training sample fails to inform \model the actual in-task knowledge~(zero retrieval in \texttt{QNLI}) and building connection between data and knowledge by a special tagged token only gives minor improvements. Instead, a well-designed knowledge prompting can actually help \model learn task-specific knowledge.


\begin{table}[htbp]
	\centering
	\resizebox{0.95\linewidth}{!}{
	\begin{tabular}{cccccc}
    \toprule[1.2pt]
    \bf Task &  \bf Ori. & \bf Concate. &\bf Tagged. &\bf Prompting.\\
    \midrule[0.5pt]
	QNLI & 91.28 & 91.28 & 91.37 & \bf 91.58 \\
	QQP  & 90.56 & 90.12 & 90.76 & \bf 91.47 \\
	\bottomrule[1.2pt]
    \end{tabular}}
    \caption{
    Performance of in-task knowledge on \texttt{QNLI} and \texttt{QQP} measured by accuracy.}
    \label{tab:in-task_knowledge}
\end{table}

\subsection{Tuning \model}
\label{sec:tuning_model}
We investigate how key design affects the performance of \model. 
(1)~\textbf{Number of Retrieved Knowledge.} Figure~\ref{fig:num_knowledge} shows the effects of different N in STS-B dataset and the sparsely activated Top-5 knowledge proves to be optimal. 
(2)~\textbf{Layers equipped with DPM.} Considering that the  upper layers in PLM capture more semantic information~\citep{geva2021transformer}, we equip the last encoder layer with DPM in \model.  Figure~\ref{fig:num_knowledge} shows that increasing DPM-enhanced encoder layer gives minor improvements but brings much latency because of extra MIPS search. 
(3)~\textbf{FFN and \memory.} To further explore the relation between FFN and \memory, we propose two model variants. First, we replace FFN in all encoder layers with a shared DPM denoted as \model$_{\text{All}}$. Then we fuse FFN and DPM by modifying the model architecture from $\text{LayerNorm}(h+\text{KnowAttn}(h,\mathbb{K}_{h'},\mathbb{V}_{h'}))$ to $\text{LayerNorm}(h+\text{KnowAttn}(h,\mathbb{K}_{h'},\mathbb{V}_{h'})+\text{FFN}(h))$ and we name it \model$_{\text{Fuse}}$. The Spearman correlation~(more results are shown in Appendix~\ref{appendix:tuning_model}) in STS-B dataset for WikiBERT, \model$_{\text{All}}$, \model and \model$_{\text{Fuse}}$ is 88.64, 86.82, 89.20 and 89.10. We could find that \model$_{\text{All}}$, where there is no FFN, underperforms WikiBERT. And \model performs comparably with \model$_{\text{Fuse}}$. We conjecture that FFN in different layers may play different roles, which is also reported in \citet{geva2021transformer}. For the upper layer which captures more semantic knowledge~\citep{jawahar2019does}, \memory is a flexible and extensible substitution of FFN, but for lower layers, shallow features should be captured in the model parameters.


\begin{figure}[thbp]
	\includegraphics[width=\linewidth,height=0.45\linewidth]{figs/number_knowledge_num_layers.pdf}
        \caption{Effect of the number of retrieved knowledge and the number of DPM-enhanced layers in \texttt{STS-B} measured by spearman correlation.}
        \label{fig:num_knowledge}	
\end{figure}





==> content/5-conclusion.tex <==
In this paper, we propose a novel knowledge encoding mechanism for PLMs, which decouples the learned knowledge during pre-training from the parameters of the PLMs. This enables the knowledge encoding of PLM more flexible and interpretable. Inspired by previous works that show FFN in Transformer acts like a key-value memory network and it is where PLMs store acquired knowledge during pre-training, we creatively use differentiable plug-in memory (DPM) to replace FFN and conduct knowledge retrieval with Maximum inner-product search in DPM, which is the first work to make such exploration. Extensive experimental results verify the flexibility and scalability of \model in various settings including domain adaptation, knowledge update and in-task knowledge learning. 

==> content/tables/case_study.tex <==
%\begin{table}[t]
%\centering	
%\resizebox{1\linewidth}{!}{
%\begin{tabular}
%    {m{2cm}m{10.5cm}cc}
%\toprule[1.5pt]
%\bf Question & \bf Answer  & \bf Prediction & \bf Label  \\
%\midrule[0.5pt]
%How much of Jacksonville is made up of water? & According to the United States Census Bureau, the city has a total area of 874.3 square miles (2,264 $\text{km}^2$), making Jacksonville the largest city in land area in the contiguous United States; of this, 86.66\% (757.7 sq mi or 1,962 $\text{km}^2$) is land and ; 13.34\% (116.7 sq mi or 302 $\text{km}^2$) is water.  & Entailment & Entailment   \\
%\midrule[0.5pt]	
%\addlinespace[0.15em]
%\bf Knowledge
%&\multicolumn{3}{|m{14.5cm}}{
%this article lists the 3, 143 states of america. the 50 states of ``... by the united states census bureau...the united states census bureau ( uscb ) , officially the bureau of the census...\% white, 9. 3 \% african american, 0.3 \% native american, 2.9 \% asian, 0.1 \% pacific islander, 0.2 \% from other races, and 3.9 \% from two or more races. hispanic or latino of any race were 6.8 \% of the population...} \\
%\bottomrule[1.5pt]
%\end{tabular}}
%\caption{Example from QNLI dataset. The knowledge is filtered for brevity. For the full example and more other examples please refer to Appendix~\ref{appendix:case_study}.}
%\label{tab:case_study}
%\end{table}
